From Instruction to Output: The Role of Prompting in Modern NLG

Prompt engineering has emerged as an integral technique for extending the strengths and abilities of Large Language Models (LLMs) to gain significant performance gains in various Natural Language Processing (NLP) tasks. This approach, which requires instructions to be composed in natural language to bring out the knowledge from LLMs in a structured way, has driven breakthroughs in various NLP tasks. Yet there is still no structured framework or coherent understanding of the varied prompt engineering methods and techniques, particularly in the field of Natural Language Generation (NLG). This survey aims to help fill that gap by outlining recent developments in prompt engineering, and their effect on different NLG tasks. It reviews recent advances in prompting methods and their impact on NLG tasks, presenting prompt design as an input-level control mechanism that complements fine-tuning and decoding approaches. The paper introduces a taxonomy of prompting paradigms, a decision framework for prompt selection based on varying factors for the practitioners, outlines emerging trends and challenges, and proposes a framework that links design, optimization, and evaluation to support more controllable and generalizable NLG.

==> humanInTheLoop.tex <==

While much of the research on prompting has focused on automated discovery or optimization, an equally important dimension concerns how humans iteratively interact with large language models (LLMs) through prompts. 
Rather than treating prompts as static inputs, recent studies have emphasized the \textit{interactive refinement process}, where users adjust phrasing, constraints, or style markers in response to model outputs. 
This perspective frames prompt engineering as a dynamic, human-in-the-loop activity rather than a one-off design problem.

Interactive prompt refinement highlights several opportunities. 
First, it enables \textbf{collaborative co-adaptation}, where users learn to craft more effective instructions while models reveal their strengths and weaknesses through feedback loops. 
Second, it supports \textbf{accessibility and usability}, with recent work exploring natural language interfaces, visual prompt editing tools, and even tactile or speech-based modalities for diverse user groups. 
Third, it aligns with the broader movement towards \textbf{human-centered AI}, recognizing that prompt design cannot be divorced from the contexts, intentions, and expertise of its users.

From a research perspective, human-in-the-loop prompting opens new questions: 
How can systems scaffold user learning of effective prompts? 
What metrics best capture interactive success (e.g., efficiency of convergence to desired output)? 
And how can participatory design approaches ensure that prompting paradigms are inclusive, particularly in multilingual or cross-cultural settings? 
Exploring these dimensions will be essential to establish prompt engineering not merely as an optimization problem, but as a socio-technical practice that bridges automation with human creativity and control.

